Compass-V2 Technical Report

Predominant LLMs focus on high-resource languages while leaving low-resource languages, particularly those in Southeast Asia (SEA), underrepresented. In addition, those models are general-purpose and pay limited attention to the e-commerce domain. To overcome these limitations, we introduce Compass-v2, a lightweight Mixture-of-Experts (MoE) model specifically designed for Southeast Asian languages and e-commerce applications. To balance model performance and inference cost, the model is designed with 30B total parameters and 5B active parameters, incorporating both fine-grained and shared expert modules. To enhance multilingual performance, we curated and constructed a high-quality, industry-leading SEA dataset, to the best of our knowledge. To boost performance in the e-commerce domain, we built a dataset comprising hundreds of billions of tokens, sourced through external data mining and internal platform collection. Besides, we pioneered a hybrid reasoning model that supports both fast thinking and deep thinking within a unified framework to enhance the reasoning capabilities, diverging from the conventional industry practice of deploying two separate models. Through extensive experimental evaluations, our model demonstrates state-of-the-art SEA multilingual and e-commerce performance among sub-30B models, while maintaining significantly lower inference cost.

==> 11_api.tex <==
\section{The Compass API Platform (CAP)} \label{chapeter:api}
In this section, we begin by first introducing the key takeaways of Compass API Platform (CAP). 
Next, we present the system designs, including the overall platform architecture, and how to call the APIs of CAP.


\subsection{Introduction}

\href{https://compass.llm.shopee.io/}{CAP} provides pre-built Compass series of Large Models, which are independently developed by Shopee. These models are designed to be seamlessly integrated into AI-powered applications, enabling businesses to leverage advanced AI capabilities without extensive development efforts.

CAP accelerates the time to market for AI applications by eliminating the need for time-consuming and resource-intensive model development and management activities. CAP offers the Compass series of Large Models as a service, also known as Model as a Service (MaaS), to enable access via APIs. This approach allows application development and deployment, while leveraging the robust infrastructure and expertise provided by Shopee.

Currently, CAP offers two distinct approaches to harness the capabilities of the Compass series of Large Models:

\begin{itemize}
    \item Through the \textbf{\href{https://compass.llm.shopee.io/chat}{Portal}} (see more details in Appendix A): Similar to ChatGPT, it is used for rapid experience and effect testing.
    \item Through the \textbf{\href{https://compass.llm.shopee.io/docs}{API}}: Used for production scenarios.
\end{itemize}

\subsection{Platform Architecture}

\begin{figure}[htbp]
    \centering
    \includegraphics[width=1\textwidth]{./figures/9_api/API_1.pdf}
    \caption{API Platform of Compass-v2}
    \label{fig:api}
\end{figure}

CAP adopts a service-oriented design \citep{service-oriented} to achieve fine-grained decoupling among the system components. As shown in Figure~\ref{fig:api}, from top to bottom, CAP has three layers: HTTP Endpoints layer, Gateway Capabilities layer, and Model Services layer.

\textbf{HTTP Endpoints} layer serves as a fundamental component by offering a standardized interface for communication between clients and the server. Specifically, CAP exposes several key endpoints for text generation, vision understanding, audio transcription, vector stores, supervised fine-tuning (work in progress), etc. 

For instance:
\begin{itemize}
    \item The \texttt{/v1/chat/completions} endpoint generates a model response based on the provided chat conversation.
    \item The \texttt{/v1/embeddings} endpoint turns text into numerical representations, enabling use cases like search.
    \item The \texttt{/v1/audio/transcriptions} endpoint facilitates the transcription of audio into the specified input language.
    \item The \texttt{/v1/files/*} endpoints are used to upload documents for features like Fine-tuning, Vector Store, and Batch API.
    \item The \texttt{/v1/batch/*} endpoints facilitate the creation and execution of batch processes using uploaded files containing multiple requests.
    \item The \texttt{/v1/vector\_stores/*} endpoints serve as a versatile tool for managing knowledge bases, processing files, and conducting semantic searches. It is particularly well-suited for applications in Retrieval-Augmented Generation (RAG) scenarios \citep{lewis2021retrievalaugmentedgenerationknowledgeintensivenlp}.
    \item The \texttt{/v1/fine\_tuning/*} endpoints, currently under development, manage fine-tuning jobs to customize a model to fit specific training data.
\end{itemize}

These endpoints are meticulously designed to adhere to RESTful principles, thereby ensuring broad compatibility with various clients and efficient data exchange. Through the clear definition and comprehensive documentation of these endpoints, CAP achieves both flexibility and scalability. This design choice not only enhances the system's adaptability to evolving requirements but also facilitates seamless integration with other services and applications, thereby fostering a more cohesive and interoperable ecosystem.

\textbf{Gateway Capabilities} layer serves as a critical component that manages all client requests by performing format validation, permission verification, traffic control, and log recording. For each endpoint, the Gateway implements specific security validation strategies and intervention policies to safeguard the integrity of user inputs and model outputs. 

Leveraging the optimization potential of KV-Caches in the Transformer architecture, the Gateway dynamically selects suitable inference instances based on the prompt prefix. This approach maximizes the utilization of the KV Cache to accelerate inference.

Furthermore, the Gateway integrates a comprehensive observability module. This module provides real-time monitoring of service quality from three critical dimensions: business metrics, technical metrics, and resource metrics. By doing so, it ensures robust performance and reliability of the entire system.

\textbf{Model Services} layer plays a pivotal role in managing GPU hardware resources and orchestrating model deployment and updates. It is designed with automatic scaling capabilities, which dynamically adjust resource allocation based on key performance metrics, including Time to First Token (TTFT), Time Per Output Token (TPOT), GPU utilization rates, etc. These metrics enable the layer to optimize resource usage in real-time, ensuring efficient and responsive system performance.

Furthermore, the model service layer is dedicated to enhancing model inference performance through advanced optimization techniques. These optimizations are specifically aimed at fully leveraging the computational capabilities of GPUs, thus maximizing inference speed and efficiency.

In addition to these functions, the model service layer implements a hybrid deployment and scheduling strategy for both offline and online inference resources. This hybrid approach allows for the effective utilization of GPU clusters, balancing the demands of real-time inference with the efficiency of batch processing. By doing so, it ensures that the overall throughput of the GPU cluster is maintained at a high level, meeting the stringent performance requirements of modern AI applications.

In general, the model service layer serves as a critical component in the CAP architecture, providing robust resource management, performance optimization, and flexible deployment strategies to support diverse AI workloads.

\subsection{API Call Example}

CAP provides OpenAI-compatible APIs to enable a smooth transition from OpenAI services to the Compass series of Large Models. A complete reference for the API is available in \href{https://compass.llm.shopee.io/docs}{Compass API Reference}. Currently, CAP’s RESTful API is compatible with the following OpenAI interfaces, with additional compatibility planned for future development:

\begin{itemize}
    \item \texttt{/v1/chat/completions}
    \item \texttt{/v1/embeddings}
    \item \texttt{/v1/audio/transcriptions}
    \item \texttt{/v1/files/*}
    \item \texttt{/v1/batches/*}
    \item \texttt{/v1/vector\_stores/*}
\end{itemize}

To generate text with Compass-v2, the chat completions endpoint (\texttt{/v1/chat/completions}) in the REST API can be used, as demonstrated in the example below. This endpoint can be accessed via an HTTP client of choice or through one of OpenAI’s official client SDKs, which are available for various programming languages.\\

\begin{lstlisting}[language=bash, breaklines=true, frame=single]
curl "http://compass.llm.shopee.io/compass-api/v1/chat/completions" \
    -H "Content-Type: application/json" \
    -H "Authorization: Bearer $COMPASS_API_KEY" \
    -d '{
        "model": "compass-v2",
        "messages": [
            {
                "role": "user",
                "content": "Write a one-sentence bedtime story about a unicorn."
            }
        ],
        "stream": true
    }'
\end{lstlisting}

The model-generated content is organized as an array within the choice attribute of the response object. In this particular example, the response contains a single output element, which is presented below.\\

\begin{lstlisting}[language=bash, breaklines=true, frame=single]
[
    {
        "index": 0,
        "message": {
            "role": "assistant",
            "content": " In a mystical forest, under the soft glow of the moon, a young unicorn named Luna ...",
            "tool_calls": null
        },
        "logprobs": null,
        "finish_reason": "stop"
    }
]
\end{lstlisting}




==> 3_posttraining_bak.tex <==
% \section{Post-Training} \label{chapter:posttraining}
% Our post-training process includes the SFT phase and the RL phase. The SFT phase enhances performance for most general QA evaluations, while the RL phase improves the model's natural tone and generalization capabilities.

\section{Supervised Fine-tuning}

\subsubsection{SFT Data}
% Now our SFT data is about 6 million data, and we get data from three channels: open source data, synthetic data, and real business data. The ratio is about 6:3:1. 
Our current SFT dataset contains approximately 6 million samples, sourced from three channels: open source data, synthetic data, and real business data, with a composition ratio of roughly 6:3:1.
% We classified the data at the task level, and divided the data into 10 categories at the first level: security, knowledge, understanding, mathematics, reasoning, creative generation, code, e-commerce, agent, and platform-related information. We further subdivided each level, with a total of 70 subcategories. 
To support robust multi-task capabilities, we organize the data at the task level into 10 first-level categories: safety, knowledge, understanding, math, reasoning, creative generation, code, e-commerce, agent, and platform-related information. These data can be further divided into 70 subcategories, enabling better coverage across diverse use cases.

% Considering the actual business needs, we have made a more detailed classification of the data at the language level, and performed language recognition at the sentence level. Sentence-level language recognition is easier to identify and filter some translations and synthetic error responses than reposne-level language recognition. 
% Our current language requirements are English, Chinese, Traditional Chinese (Taiwan), Filipino, Malay, Indonesian, Portuguese, Vietnamese, and Thai.
Given our model's deployment in the multilingual Southeast Asian market, our SFT dataset contains a diverse set of languages, including English(en), Chinese(zh), Tagalog(tl), Malay(my), Indonesian(id), Portuguese(pt), Vietnamese(vi), and Thai(th). 
To ensure accurate language labeling, we apply sentence-level language identification rather than response-level identification. This allows us to filter out noisy translations and synthetic responses more effectively, thereby improving the overall quality of our SFT dataset.

% \begin{figure}[h]
%     \centering
%     \begin{minipage}{0.48\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{./figures/3_posttraining/lang.pdf}
%         \caption{SFT data language distribution}
%     \end{minipage}\hfill
%     \begin{minipage}{0.48\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{./figures/3_posttraining/task.pdf}
%         \caption{SFT data task distribution}
%     \end{minipage}
% \end{figure}



%
% We conducted comprehensive filtering of the SFT data, dividing the process into four main parts:
We conducted a comprehensive multi-stage filtering process for the SFT dataset, dividing it into four key components:
\begin{itemize}
    \item \textbf{Heuristic Filtering}: 
    % We used rules to filter out a portion of obviously dirty data and employed heuristic rules to cover as much dirty data as possible.
    We applied a set of heuristics rules to filter out low-quality or corrupted data. These rules were designed to cover a wide range of noisy patterns, helping to efficiently remove low-quality data at scale.

    \item \textbf{Embedding clustering}: 
    % We applied embedding clustering to filter out some similar data, prioritizing data from diverse sources in the open-source datasets to ensure variety in data origins.
    We applied embedding clustering to filter out highly similar samples. To maintain data diversity and maximize data coverage, we prioritize data selection from diverse sources.

    \item \textbf{LLM-based filtering}: 
    % We used GPT-4 to filter the prompts and responses in the existing data. Our criteria for prompts were clarity of language, absence of obvious formatting issues, and no ambiguous special symbols. For responses, our filtering standards included strict adherence to instructions, and for certain tasks, we removed responses that were not in Markdown format to ensure readability.
    We used GPT-4 to filter out the low-quality prompts and responses. For prompts, our filtering criteria consist of language clarity, formatting errors, and ambiguous special characters. For responses, we emphasized on instruction adherence and removed responses with incorrect formats (e.g, non-Markdown answers in certain tasks, leading to bad readability).

    \item \textbf{Human annotation}: 
    % We implemented manual validation to verify part of the synthetic data. For each data entry, we used three human annotators, and only data approved by all three was included in the final dataset.
    We conducted manual validation to ensure the quality of our synthetic data. Each selected synthetic sample was reviewed by three human annotators, and only those approved by all three were retained in the final dataset.
\end{itemize}
In the following sections, we provide detailed explanations and examples for each category of our SFT data. 
\begin{figure}[h]
    \centering
    \begin{minipage}{0.98\textwidth}
        \centering
        \includegraphics[width=\textwidth]{./figures/3_posttraining/sft_weiwei.pdf}
        \caption{SFT data process pipeline}
    \end{minipage}
\end{figure}
\paragraph{Hard instruction following} In enhancing the instruction-following capability of large language models, data quality is critical. We employ two key strategies: data filtering and data synthesis to ensure that the model can comprehend and strictly adhere to diverse instruction constraints. First, during the data filtering stage, we ensure that the selected data exhibits sufficient instruction diversity, covering various task types (such as Q\&A, summarization, code generation, and text rewriting) and instructions of different complexity levels. This diversity helps the model learn instruction execution patterns across different contexts. Second, in the data synthesis stage, we leverage advanced models like GPT-4o and DeepSeek-R1 as data generators to produce high-quality example responses. We place special emphasis on verifiable precise instruction data, where the instructions explicitly specify constraints such as output length, format, language, tone, options, and keywords. 

By incorporating such fine-grained constraints, we can construct a large volume of high-quality training data, allowing the target model to become accustomed to following detailed instructions precisely. Furthermore, this data can be used for automated evaluation to ensure the model’s controllability and consistency in instruction execution. Ultimately, through the above data filtering and synthesis strategies, we can significantly improve the instruction-following capability of large language models, enabling them to maintain high accuracy and consistency even when handling complex instructions.

\input{./content/e-commerce}

\input{./content/agent}

\input{./content/multilingual}

\input{./content/subjective_synthetic_data}
% \subsubsection{Training Setting}
% pass


\subsection{Two Stages Training for SFT}

In our latest experiment on large-scale Supervised Fine-Tuning (SFT), we designed a two-stage training strategy to develop a model that not only follows general instructions but also demonstrates deep reasoning abilities and strong e-commerce and multilingual capabilities. Balancing these aspects posed significant challenges, requiring careful data selection and curriculum design.

In the \textbf{first stage}, we focused on establishing strong generalization and instruction-following capabilities. The model was fine-tuned on a diverse dataset covering various domains, including information processing, commonsense QA, text generation, coding, logical reasoning, STEM, and safety-related tasks. This foundational phase enabled the model to understand and execute a broad range of instructions effectively.

In the \textbf{second stage}, we introduced additional targeted datasets to refine reasoning abilities and domain expertise:

\begin{itemize}
    \item \textbf{Mathematical reasoning data}: We incorporated problem-solving datasets with explicit thought processes wrapped in <think></think> tags, enhancing the model's ability to generate structured, multi-step solutions.

    \item \textbf{Selective resampling of high-quality data}: To maintain distributional alignment with the first stage, we sampled high-quality instruction data across multiple domains and integrated it into this phase.
    
    \item \textbf{Expanded reasoning steps}: A subset of first-stage data, particularly multiple-choice questions (A/B/C/D), was enhanced with detailed step-by-step explanations to improve logical inference.
    
    \item \textbf{E-commerce data augmentation}: Specialized datasets focusing on product descriptions, customer inquiries, and transactional reasoning were added to strengthen the model’s ability in e-commerce-related tasks.
    
    \item \textbf{Role-playing and function-calling tasks}: To improve adaptability in interactive and API-driven applications, we incorporated data for role-based conversations and function execution.
\end{itemize}

Our results indicate that this mixed-training approach effectively combines general instruction-following with advanced reasoning capabilities. The model not only excels in complex mathematical reasoning tasks, such as MATH-500, but also demonstrates deeper logical thinking in general inference tasks. By structuring the training in this manner, we successfully developed a model capable of both general instruction execution and advanced multi-step reasoning, while also enhancing its performance in e-commerce and multilingual scenarios.
Our training process was conducted in two stages using 24 H100 GPUs. In the first stage, we trained the model with 9.8 million data samples, followed by a second stage with 480,000 samples. The maximum learning rate was set to \(3 \times10^{-5} \), which was gradually decayed to zero using a cosine schedule. The warmup ratio was configured as 0.02 to ensure stable early-stage training.


For batch settings, we used a micro-batch size of 1 with a gradient accumulation step of 4. Additionally, to prevent errors in loss computation caused by gradient accumulation, the loss was averaged across the sample dimension within the global batch. This adjustment ensured more accurate gradient updates while maintaining training stability.

\subsection{Implementation of Full Parameters Training Framework}
When selecting a framework for post-training, we compared the performance of several frameworks suitable for instruction fine-tuning, including Transformers, LLaMA-Factory, and OpenChat. Although these frameworks meet the basic requirements for post-training, due to the large parameter size of the model and considering subsequent training efficiency issues, using only the DP (Data Parallel) mode from these frameworks for training introduces more communication overhead and leads to insufficient utilization of GPU resources. Therefore, we constructed a post-training framework based on Megatron-LM.

We initially attempted to incorporate MASK tensors as additional input information to the framework, which would allow us to build the framework with minimal modifications. However, since post-training focuses more on sample integrity and variability in token counts per sample compared to pre-training, this approach introduced more pad tokens, significantly reducing the proportion of effective computation.

Subsequently, we tried using a dynamic padding strategy to ensure that all input tokens were effective. However, this caused a noticeable decrease in overall training speed (similar to issues mentioned in FSDP research). Therefore, we implemented Distributed Dynamic Padding (DDP), which ensures consistent input sizes for each DP group (despite some efficiency loss), resulting in speeds more in line with expectations. In practice, however, these variable-length inputs often caused experiments to be interrupted due to communication issues.

Finally, based on requirements for sample integrity during post-training, training speed, training stability, and precision of the Megatron-LM-based post-training framework, we implemented a sample packing operation (similar to OpenChat). This allows for training more samples in a single forward/backward pass with the same batch size. We also improved the communication strategies of existing parallelization methods to adapt to this training mode. We compared the speed and precision of our new framework with existing frameworks and found that, under similar configurations, the new framework is tens of percent faster than the previously mentioned frameworks, while the average difference in step loss during training between our framework and the others does not exceed three decimal places.


\subsection{Tips for training}

To investigate the importance of different model components during the SFT training process, we selected approximately 20,000 domain-specific data samples and analyzed the train loss at the third epoch. This evaluation aimed to assess whether the model could approximate the fitting capability of full-parameter fine-tuning. We employed layer freezing techniques to control which parts of the model remained trainable.

Specifically, we conducted experiments where different sets of parameters were selectively trained, including: (1) the full parameters of the first and last $N$ layers, (2) the MLP components, (3) the non-gate sections, and (4) the self-attention modules. The detailed results, as presented in Table~\ref{tab:training_results of sft module}, show a strong alignment with our previous findings on dense models. Our key conclusions are as follows:
\begin{itemize}
\item The last $N$ layers require more training than the first $N$ layers.
\item The MLP layers are more critical for training than the self-attention layers.
\item During the second phase (S2) of training, the gate in the MLP layers can be selectively frozen.
\item For downstream tasks, the choice of which module to prioritize for training can be adjusted based on the parameter capacity of the available training hardware.
\end{itemize}

These insights provide a clearer understanding of structural sensitivity, contributing to better optimization strategies for future model fine-tuning.

\begin{table}[h]
    \centering
    \begin{tabular}{lccr}
        \toprule
        \textbf{Setting} & \textbf{Loss} & \textbf{Trainable Module} & \textbf{Trainable Params} \\
        \midrule
        Full & 0.1561 & Full Paramaters & 30B \\
        \midrule
        Freeze-1 & 0.49945 & Last 2 layers full-parameter & 2.99B \\
        Freeze-2 & 0.41901 & Last 4 layers full-parameter & 5.83B \\
        Freeze-3 & 0.47148 & First 4 layers full-parameter & 5.83B \\
        Freeze-4 & 0.51233 & up\_proj, down\_proj of last 8 layers & 3B \\
        Freeze-5 & 0.31789 & Last 8 layers full-parameter & 11B \\
        Freeze-6 & 0.47483 & gate\_proj, up\_proj, down\_proj of last 8 layers & 4.5B \\
        Freeze-7 & 0.60042 & Self\_attention of last 8 layers & 0.18B \\
        \midrule
        LoRA-1 & 0.45686 & rank=256, applied to all layers & 6B \\
        LoRA-2 & 0.38524 & rank=512, applied to MLP in all layers & 11B \\
        \bottomrule
    \end{tabular}
    \caption{Training Settings and Loss Comparison}
    \label{tab:training_results of sft module}
\end{table}



\section{Reinforcement Learning}

\subsection{Reward modelling}
\input{./content/reward_model}

\subsection{Online Reinforcement Learning}
\input{./content/rlhf}















==> agent.tex <==
\textbf{Function Calling Data} We curate a function calling data of 154{,}563 raw prompt-response pairs, each optionally annotated with a \texttt{tools} field containing structured metadata on tool usage. To support supervised training and evaluation, we prioritize entries with non-empty \texttt{tools} fields, selecting for diversity in tool schemas and argument complexity to ensure broad coverage and improve generalization. Of the raw entries, 34{,}597 lack tool annotations, indicating no tool was invoked; while not directly informative for modeling tool semantics, these examples serve as negative cases to help the model discriminate between invocation and non-invocation prompts. The resulting dataset balances tool coverage and contrast, making it suitable for fine-tuning on structured function calling tasks and for evaluating generalization to varied tool interfaces.

\textbf{Question Answering Data} We curate a high-quality question answering dataset derived from HotpotQA~\citep{yang2018hotpotqa}, systematically reformulating instances along four key dimensions inspired by~\citep{chen2023benchmarking}: contextual noise resilience, negative rejection, information integration, and counterfactual stability. a) For contextual noise resilience, we introduce lexically relevant but semantically irrelevant distractors into the retrieved context, assessing the model’s ability to isolate pertinent evidence from spurious content. 2) For negative rejection, we include queries for which no supporting evidence is present in the retrieved passages, encouraging the model to refrain from answering in the absence of sufficient grounding rather than defaulting to hallucinated responses. 3) For information integration, questions require the aggregation of complementary information scattered across multiple documents. 4) Counterfactual stability is assessed by injecting fabricated or contradictory statements into the context, measuring the model’s sensitivity to misinformation and its ability to preserve factual consistency. To support broad generalization, the dataset includes questions spanning a range of difficulties and evidence configurations, encouraging more reliable and interpretable performance in open-domain QA settings.

\textbf{Coding Data} To enhance the model's coding capabilities, we construct an instruction-tuning coding corpus encompassing nearly 40 programming languages by integrating open-source data with domain-specific synthetic data. Our dataset covers a broad spectrum of topics and instruction types, ranging from algorithmic problem-solving to package-specific knowledge, and includes tasks such as conventional Q\&A, code completion, test case generation, and code refinement. These diverse elements provide comprehensive coverage of both theoretical and practical programming aspects, spanning various difficulty levels from foundational exercises to advanced competitive coding challenges. To further improve data quality, a subset of the dataset undergoes unit testing, enhancing reliability and ensuring instructional coherence and code correctness.

\textbf{Role-playing Data} We construct a role-playing dataset by combining open-domain corpora~\citep{li2023chatharuhirevivinganimecharacter, wang2025coser} with synthetic dialogues generated via instruction-tuned LLMs. To broaden representational diversity, the dataset integrates two complementary dialogue settings: authentic conversations between real-world characters extracted from books and fictional interactions involving synthetic personas in imagined scenarios. The former provides authentic and context-rich exchanges that preserve narrative coherence and character consistency, while the latter enables controlled expansion into underrepresented roles, dialogue intents, and stylistic modes. Redundancy is mitigated through character-level deduplication based on identity and scene similarity. Synthetic dialogues are generated using structured character profiles encoding identity, background knowledge, and stylistic attributes; these profiles inform prompt construction to ensure linguistic and contextual consistency in generated interactions. The system prompt schema is detailed in Table~\ref{tab:roleplay_prompt_design}.


\begin{table}[h!]
    \centering
    \begin{tabular}{p{12cm}}
    \toprule
    \textbf{System Prompt for Role-playing} \\
    \hline
    I want you to act like \{character\}. I want you to respond and answer using the tone, manner and vocabulary that would be appropriate, using all relevant knowledge for this \{character\} in English/Chinese. \\
    \vspace{1em}
    Character Name: \\
    \{character\} (Necessary) \\
    \vspace{1em}
    The context is as follows: \\
    \{context\} (if available) \\
    \vspace{1em}
    The profile of \{character\} is as follows: \\
    \{character\_profile\} (if available) \\
    \vspace{1em}
    Here is your knowledge about the other characters: \\
    \{other\_character\_profiles\_str\} (if available) \\
    \vspace{1em}
    Other restrictions: \\
    \{other\_restrictions\} (if available) \\
    \vspace{1em}
    The Current Scenario is as follows: \\
    Location: \\ \{location\} (if available) \\
    Status: \\ \{Status\} (if available) \\
    \bottomrule
    \end{tabular}
    \caption{Prompts for role-playing dataset construction}
    \label{tab:roleplay_prompt_design}
\end{table}

==> longcot.tex <==
\textbf{Long-CoT Data} To enhance reasoning capabilities, we introduce a Long Chain-of-Thought data with thinking process and summarized answer to make Compass as a Mixed-Reasoning-Model. We began by collecting a diverse range of sources of math queries with groundtruth answers as seed set (e.g. NuminaMath\cite{numina_math_datasets}, LIMO\cite{ye2025limoreasoning},S1K-1.1\cite{muennighoff2025s1simpletesttimescaling}). We implement data deduplication with exact matching and thorough decontamination against MATH500,AIME24,AIME25 and GPQA. The data is then filtered for complexity and response length, where we initially employ previous Compass-v2 model to rollout responses several times for collected queries. Math-Verify is applied to retrieve correct examples. Queries with a pass rate that falls within the interval [$\alpha$, $\beta$] are selected, where the process helped set an initial difficulty threshold to filter out exceptionally challenging or trivial problems. Downsampling strategy is leveraged to balance the capabilities between general and reasoning.

==> tables/inference_evaluation.tex <==
\begin{table}[]

\centering
\caption{ Evaluation on standard benchmarks using the Compass-v2 API. FP8 and AWQ-INT4 quantization approach has negligible impact on the model’s quality.
}
\resizebox{\columnwidth}{!}{
\begin{tabular}{@{}cccccc@{}l}

\toprule
\textbf{}            & \textbf{Reasoning} & \textbf{Question Answer} & \textbf{Reading Comprehension} &  \textbf{Safety} &\textbf{Math}  \\ \midrule
Compass-v2-FP16&  0.7060&   0.8392& 0.8859  & 0.5149& 0.2932  \\ 
Compass-v2-FP8& 0.7055&   0.8304&   0.8838 & 0.5011&  0.2924  \\ 
Compass-v2-AWQ-INT4& 0.6987& 0.8312& 0.8823    & 0.5330& 0.2874    \\ 
\bottomrule
\end{tabular}
}

% \vspace{-0.2cm} % 减少图片下方的间距
\label{Table:Evaluations on standard benchmarks with inference API}
\end{table}

==> tables/inference_open_models.tex <==
\begin{table}[]

\centering
\caption{  Evaluations on standard benchmarks with inference API. FP8 and AWQ-INT4 quantization approach has negligible impact on the model’s quality.
}
\resizebox{\columnwidth}{!}{
\begin{tabular}{@{}ccccccc@{}l}

\toprule
\textbf{}            & \textbf{Reasoning} & \textbf{Question Answer} & \textbf{Reading Comprehension} &  \textbf{Safety} &\textbf{Math}   &\textbf{Multilingual}\\ \midrule
Compass v2-FP16&  0.7060&   0.8392& 0.5005  & 0.5149& 0.2932 &0.4878 \\ 
Compass v2-FP8& 0.6987&   0.8312&   0.4718 & 0.5330&  0.2924 &0.6402 \\ 
Compass v2-AWQ-INT4& 0.7055& 0.8304& 0.4459    & 0.5011& 0.2874 &0.4476    \\ 
\bottomrule
\end{tabular}
}

% \vspace{-0.2cm} % 减少图片下方的间距
\label{Table:Evaluations on standard benchmarks with inference API}
\end{table}

==> tables/pre-training_performance_evaluation_results.tex <==
\begin{table}[]

\centering
\caption{ Pre-Training Performance Evaluation Results. Compass-v2 demonstrates strong capabilities in comprehension and safety.}
\resizebox{\columnwidth}{!}{
\begin{tabular}{@{}ccccccc@{}}
\toprule
\textbf{}            & \textbf{Reasoning} & \textbf{Question Answer} & \textbf{Reading Comprehension} &  \textbf{Safety} & \textbf{Code} &\textbf{Math}  \\ \midrule
Dataset & MMLU  & GPQA  & RACE  & Jailbreak & HumanEval & MathQA   \\ \midrule
Compass-v2  &  0.6830   &   0.3687  & 0.4641  & 0.9046 & 0.4634 & 0.4171  \\
Qwen-2.5-14b       & 0.7973   &   0.3737     &   0.4105 & 0.9084   & 0.5488 &  0.5179  \\
LLaMa-3-8b  & 0.6538    & 0.303 & 0.3943    & 0.7710    & 0.3476    & 0.3963    \\

\bottomrule
\end{tabular}
}

% \vspace{-0.2cm} % 减少图片下方的间距
\label{Table:Pre-Training_Results}
\end{table}



